Solving Diophantine Equations

In this book a multitude of Diophantine equations and their partial or complete solutions are presented. How should we solve, for example, the equation {\eta}({\pi}(x)) = {\pi}({\eta}(x)), where {\eta} is the Smarandache function and {\pi} is Riemann function of counting the number of primes up to x, in the set of natural numbers? If an analytical method is not available, an idea would be to recall the empirical search for solutions. We establish a domain of searching for the solutions and then we check all possible situations, and of course we retain among them only those solutions that verify our equation. In other words, we say that the equation does not have solutions in the search domain, or the equation has n solutions in this domain. This mode of solving is called partial resolution. Partially solving a Diophantine equation may be a good start for a complete solving of the problem. The authors have identified 62 Diophantine equations that impose such approach and they partially solved them. For an efficient resolution it was necessarily that they have constructed many useful tools for partially solving the Diophantine equations into a reasonable time. The computer programs as tools were written in Mathcad, because this is a good mathematical software where many mathematical functions are implemented. Transposing the programs into another computer language is facile, and such algorithms can be turned to account on other calculation systems with various processors.

==> Conclusions.tex <==
\chapter{Conclusions}

We, the authors, hope that this book offers a valuable insight into a fascinating range of Number Theory problems. The approaches and algorithms proposed are not intended to just solve proposed problems, but also to inspire the reader to find better, more efficient or more beautiful solutions that further enrich our understanding of this field of mathematics.

The "partial results" of over $62~\eta$--Diophantine equations presented in the last chapter could prove to be an excellent starting point for anyone motivated to explore more solutions. By simply running the proposed programs and algorithms on machines with better hardware capabilities, one can extend the set numbers that verify this equations. The mathematicians interested in analytical solutions are encouraged to explore Chapter 6 where, various analytical approaches into solving Diophantine equations are presented. At the same time, students or researchers unfamiliar with the details of such mathematical problems will discover, in the first five chapters some of the most important concepts, algorithms and tools to help them in their quest to learn about Diophantine equations.

The content of this book is a result of our collective mathematical and computing expertise. While the choice of the problems is a subjective one, our intent was to cover the most interesting Diophantine equations involving Smarandache's function $\eta$. We encourage anyone to approach us with comments and observation regarding the content of this book and also with other fresh problems related to it.



==> Cover4.tex <==
\chapter*{}

In this book a multitude of Diophantine equations and their partial or complete solutions are presented. How should we solve, for example, the equation $\eta(\pi(x))=\pi(\eta(x))$, where $\eta$ is the Smarandache function and $\pi$ is Riemann function of counting the number of primes up to $x$, in the set of natural numbers?

If an analytical method is not available, an idea would be to recall the empirical search for solutions. We establish a domain of searching for the solutions and then we check all possible situations, and of course we retain among them only those solutions that verify our equation.

In other words, we say that the equation does not have solutions in the search domain, or the equation has $n$ solutions in this domain. This mode of solving is called partial resolution. Partially solving a Diophantine equation may be a good start for a complete solving of the problem.

The authors have identified 62 Diophantine equations that impose such approach and they partially solved them. For an efficient resolution it was necessarily that they have constructed many useful "tools" for partially solving the Diophantine equations into a reasonable time.

The computer programs as tools were written in Mathcad, because this is a good mathematical software where many mathematical functions are implemented. Transposing the programs into another computer language is facile, and such algorithms can be turned to account on other calculation systems with various processors.



==> Indexe_engl.tex <==
\chapter{Indexes}\label{Index}

\section{Index of notations}\label{IndexNotatii}
\small\begin{description}
  \item $\Na=\set{0,1,2,\ldots}$;
  \item $\Ns=\Na\setminus\set{0}=\set{1,2,\ldots}$;
  \item $\Int=\set{\ldots,-2,-1,0,1,2,\ldots}$;
  \item $\I{s}=\set{1,2,\ldots,s}$ : the set of indexes;
  \item $\mathbb{Q}=\set{\frac{p}{q}\ \mid\ p,q\in\Int,\ q\neq0}$ ;
  \item $\Real$ : the real numbers;
  \item $\pi(x)$ : the number of prime numbers up to $x$;
  \item $\pi_m(x)$ : the function which is the lower bound of function $\pi(x)$;
  \item $\pi_M(x)$ : the function which is the upper bound of function $\pi(x)$;
  \item $[x]$ : the integer part of number $x$;
  \item $\{x\}$ : the fractional part of $x$;
  \item $\sigma_k(n)$ : the sum of the powers of order $k$ of the divisors of $n$;
  \item $\sigma(n)$ : the sum of the divisors of $n$; $\sigma(n)=\sigma_1(n)$;
  \item $s(n)$ : the sum of the divisors of $n$ without $n$; $s(n)=\sigma(n)-n$;
  \item $\lfloor a\rfloor$ : the lower integer part of $a$; the greatest integer, smaller than $a$;
  \item $\lceil a\rceil$ : the upper integer part of $a$; the smallest integer, greater than $a$;
  \item $n\mid m$ : $n$ divides $m$;
  \item $n\nmid m$ : $n$ does not divide $m$;
  \item $(m,n)$ : the greatest common divisor of $m$ and $n$; $(m,n)=gcd(m,n)$;
  \item $[m,n]$ : the smallest common multiple of $m$ and $n$; $[m,n]=lcd(m,n)$;
  \item $\set{n_1,n_2,\ldots,n_m}^k$ : the cartesian product $k\ times$
  \begin{multline*}
    \set{n_1,n_2,\ldots,n_m}^k\\
    =\underbrace{\set{n_1,n_2,\ldots,n_m}\times\set{n_1,n_2,\ldots,n_m}\times\ldots\times\set{n_1,n_2,\ldots,n_m}}_{k\ ori} \\
    =\left\{\left(\underbrace{n_1,n_1,\ldots,n_1}_{k\ elemente}\right), \left(\underbrace{n_1,n_1,\ldots,n_2}_{k\ elemente}\right), \ldots,
     \left(\underbrace{n_1,n_1,\ldots,n_m}_{k\ elemente}\right),\right.\\
     \left.\left(\underbrace{n_1,n_1,\ldots,n_2,n_1}_{k\ elemente}\right), \left(\underbrace{n_1,n_1,\ldots,n_2,n_2}_{k\ elemente}\right), \ldots\right.\\
     \left.\ldots, \left(\underbrace{n_m,n_m,\ldots,n_m}_{k\ elemente}\right)\right\}~;
  \end{multline*}
  \item $\abs{f(x)}$ : the module or the absolute value of $f(x)$;
  \item $f(x)\equiv g(x)$ : $f$ is asymptotic to $g$ if
  \[
   \frac{f(x)}{g(x)}\to1\ \ \textnormal{when}\ \ x\to\infty~;
  \]
  \item $f(x)=o\big(g(x)\big)$ :
  \[
   \frac{f(x)}{g(x)}\to0\ \ \textnormal{when}\ \ x\to\infty~;
  \]
  \item $f(x)=O\big(g(x)\big)$ : there exists a constant $c$ such that $\abs{f(x)}<c\cdot g(x)$, for all $x$; this property is also denoted $f(x)\ll g(x)$;
\end{description}

\newpage
\section{Mathcad functions}

\begin{description}
  \item $augment(M,N)$ : concatenates matrices $M$ and $N$ that have the same number of lines;
  \item $ceil(x)$ : the upper integer part function;
  \item $cols(M)$ : the number of columns of matrix $M$;
  \item $eigenvals(M)$ : the eigenvalues of matrix $M$;
  \item $eigenvec(M,\lambda)$ : the eigenvector of matrix $M$ relative to the eigenvalue $\lambda$;
  \item $eigenvecs(M)$ : the matrix of the eigenvectors of matrix $M$;
  \item $n\ factor\rightarrow$ : symbolic computation function that factorizes $n$;
  \item $floor(x)$ : the lower integer part function;
  \item $gcd(n_1,n_2,\ldots)$ : the function which computes the greatest common divisor of $n_1,n_2,\ldots$;
  \item $last(v)$ : the last index of vector $v$;
  \item $lcm(n_1,n_2,\ldots)$ : the function which computes the smallest common multiple of $n_1,n_2,\ldots$;
  \item $max(v)$ : the maximum of vector $v$;
  \item $min(v)$ : the minimum of vector $v$;
  \item $mod(m,n)$ : the rest of the division of $m$ by $n$;
  \item $ORIGIN$ : the variable dedicated to the origin of indexes, $0$ being an implicit value;
  \item $rref(M)$ : determines the matrix \emph{row-reduced echelon form};
  \item $rows(M)$ : the number of lines of matrix $M$;
  \item $solve$ : the function of symbolic solving the equations;
  \item $stack(M,N)$ : concatenates matrices $M$ and $N$ that have the same care number of columns;
  \item $submatrix(M,k_r,j_r,k_c,j_c)$ : extracts from matrix $M$, from line $k_r$ to line $j_r$ and from column $k_c$ to column $j_c$,
  a submatrix;
  \item $trunc(x)$ : the truncation function;
  \item $\sum v$ : the function that sums the components of vector $v$~.
\end{description}

\renewcommand\indexname{{\LARGE Index of name}}
\addcontentsline{toc}{section}{Index of name}\label{IndexNume}
{\small\printindex}


==> Introducere.tex <==
\chapter{Introduction}

%Prin ecua'tie liniar'a diofantic'a se 'in'telege o ecua'tie de forma $ax+by=c$ unde $a,b,c\in\Int$ iar solu'tiile $x$ 'si $y$ sunt numere 'intregi. Aceste ecua'tii pot fi rezolvate complet, prin cunoscutul algoritm ce a fost construit de Brahmagupta\index{Brahmagupta} \citep{WeissteinDiophantineEquation}.
A Diophantine equation is a linear equation $ax+by=c$ where $a,b,c\in\Int$ and the solutions $x$ and  $y$ are also integer numbers. This equation can be completely solved by the well known algorithm proposed by Brahmagupta\index{Brahmagupta} \citep{WeissteinDiophantineEquation}.

%Hilbert\index{Hilbert D.} s-a 'intrebat 'in anul 1900 dac'a exist'a un algoritm universal pentru ecua'tia liniar'a diofantic'a. Se 'stie c'a un astfel de algoritm nu exist'a pentru solu'tia de prim ordin a ecua'tiei diofantice, lucru demonstrat de  \cite{Matiyasevich1970}\index{Matiyasevich Y. V.}.
In 1900, Hilbert\index{Hilbert D.} wondered if there is an universal algorithm that solves the Diophantine equation, but \cite{Matiyasevich1970}\index{Matiyasevich Y. V.} proved that such an algorithm does not exist for the first order solution. 

%Func'tia $\eta$ asociaz'a fiec'arui num'ar natural $n$ pe cel mai mic num'ar natural $m$ care are proprietatea c'a $m!$ este multiplu lui $n$. 'In aceast'a carte ne propunem s'a rezolv'am analitic sau empiric ecua'tii diofantice 'si ecua'tii $\eta$--diofantice adic'a ecua'tii diofantice 'in care este implicat'a func'tia $\eta$ a lui \cite{Smarandache1980a}\index{Smarandache F.}.
The function $\eta$ relates to each natural number $n$ the smalles natural number $m$ such that $m!$ is a multiple of $n$. In this book we aim to find analytical or empirical solutions to Diophantine and $\eta$--Diophantine equation, namely Diophantine equation that contain the \cite{Smarandache1980a}\index{Smarandache F.}'s  $\eta$ function.

%Prin rezolvare analitic'a 'in'telegem s'a d'am solu'tia general'a a ecua'tiei diofantice, solu'tie ce rezolv'a complect problema. Spre exemplu ecua'tia $a\cdot x-b\cdot y=c$, cu $a,b,c\in\Ns$, are solu'tia general'a $x_k=b\cdot k+x_0$ 'si $y_k=a\cdot k+y_0$, unde $(x_0,y_0)$ este o solu'tie particular'a a ecua'tiei, iar $k$ este un 'intreg, $k\ge\max\set{\lceil-x_0/b\rceil,\lceil-y_0/a\rceil}$.
An analytical solution implies a general solution that completely solves the problem. For example, the general solution for the equation $a\cdot x-b\cdot y=c$, with $a,b,c\in\Ns$ is $x_k=b\cdot k+x_0$ and $y_k=a\cdot k+y_0$, where $(x_0,y_0)$ is a particular solution, and $k$ is an integer, $k\ge\max\set{\lceil-x_0/b\rceil,\lceil-y_0/a\rceil}$.

%Prin rezolvare empiric'a 'in'telegem un set de algoritmi (de programe) care determin'a solu'tiile ecua'tiei diofantice dintr-o re'tea m'arginit'a de puncte cu coordonate numere 'intregi, numit'a de noi \emph{domeniu de c'autare} de dimensiune $d$. De exemplu, pentru ecu'tia $\eta$--diofantic'a $\eta(m\cdot x+n)=x$ pe un \emph{domeniu de c'autare} posibil, de dimensiune $d=3$, solu'tiile ar putea fi tripletele $(m,n,x)\in D_c=\set{1,2,\ldots,1000}\times\set{1,2,\ldots1000}\times\set{1,2,\ldots,999}$.
By and empirical solution we understand a set of algorithms that determine the solutions of the Diophantine equation within a finite domain of integer numbers, dubbed \emph{the search domain} fo dimension $d$. For example, the $\eta$--Diophantine equation $\eta(m\cdot x+n)=x$ over the valid \emph{search domain} of dimension $d=3$, the solutions could be the triplets $(m,n,x)\in D_c=\set{1,2,\ldots,1000}\times\set{1,2,\ldots1000}\times\set{1,2,\ldots,999}$.

%'In primul capitol s-au prezentat sec'tiuni referitoare la numere prime, teste de primalitate, algoritmi de descompunere 'in factori primi a numerelor naturale, modalit'a'ti de num'arare a numerelor prime p\^{a}n'a la num'ar $x\in\Real$. Toate acestea fiind necesare pentru rezolvarea empiric'a a ecua'tiilor $\eta$--diofantice.
The first chapter introduces concepts about prime numbers, primality tests, decomposition algorithms for natural numbers, counting algorithms for all natural numbers up to a real one, etc. This concepts are fundamental for validating the empirical solutions of the $\eta$--Diophantine equations.

%'In capitolul 2 s-a definit func'tia $\eta$ 'si propriet'a'tile cunoscute p\^{a}n'a la aceast'a or'a. Toate acestea au fost necesare pentru a prezenta algoritmul \cite{Kempner1918}\index{Kempner A. J.}, de calcul al func'tiei $\eta$. 'In finalul capitolului s-a dat secven'ta de comenzi prin care se genereaz'a fi'sierul $\eta.prn$ care con'tine valorile $\eta(n)$ pentru $n=1,2,\ldots,10^6$.
The second chapter introduces the function $\eta$ along side its known properties. This concepts allow the description of \cite{Kempner1918}\index{Kempner A. J.} algorithm that computes the $\eta$ function. The latter sections contain the set of commands and instructions that generate the file $\eta.prn$ which contains the $\eta(n)$ values for $n=1,2,\ldots,10^6$.

%'In capitolul 3 s-au prezentat func'tiile divizor $\sigma_0$, $\sigma_1$, notat'a de obicei $\sigma$, $\sigma_2$ 'si $s$. Func'tia $\sigma_0(n)$ num'ar'a num'arul de divizori a lui $n$. Valoarea func'tiei $\sigma(n)=\sigma_1(n)$ este egal'a cu suma divizorilor lui $n$. Valoarea func'tiei $\sigma_2(n)$ este egal'a cu suma divizorilor la p'atrat 'si 'in general valoarea func'tiei $\sigma_k(n)$ este egal'a cu suma divizorilor la puterea $k$. Divizori lui $n$ sunt considera'ti numerele naturale care divid pe $n$ 'incluz\^{a}nd pe $1$ 'si pe $n$. Prin urmare divizorii proprii ai lui $n$ sunt to'ti divizorii f'ar'a $n$. Atunci func'tia $s(n)=\sigma(n)-n$ este, de fapt, suma divizorilor proprii. Pe l\^{a}ng'a aceste defini'tii sunt prezentate propriet'a'tiile 'si algoritmi de calcul al acestor func'tii. Cu ajutorul acestor algoritmi (programe) s-au generat fi'sierele $\sigma0.prn$, $\sigma1.prn$, $\sigma2.prn$, $s.prn$ care con'tin toate valorile func'tiilor $\sigma_0(n)$, $\sigma(n)$, $\sigma_2(n)$ 'si $s(n)$ pentru $n=1,2,\ldots,10^6$. 'In acest capitol am alocat o sec'tiune numerelor $k$--perfecte.
The third chapter describes the division functions $\sigma_0$, $\sigma_1$, usually denoted by $\sigma$, $\sigma_2$ 'si $s$. The $\sigma_0(n)$ function counts the number of divisors of $n$, while $\sigma(n)=\sigma_1(n)$ returns the sun of all those divisors. Consequently $\sigma_2(n)$ computed the sum of squared divisors of $n$ while, in general $\sigma_k(n)$ add all divisors to the power of $k$. We call divisors of $n$ all natural numbers that divide $n$ including $1$ and $n$, thus the proper divisors are considered all natural divisors excluding $n$ itself. In this case the function $s(n)=\sigma(n)-n$ is , in fact, the sun of all proper divisors. Along side the the definition, this third chapter also contains the properties and computing algorithms that generate the files $\sigma0.prn$, $\sigma1.prn$, $\sigma2.prn$, $s.prn$ that contain all the values for functions $\sigma_0(n)$, $\sigma(n)$, $\sigma_2(n)$ and $s(n)$ for $n=1,2,\ldots,10^6$. The last section describes the $k$--perfect numbers.

%Capitolul 4 trateaz'a func'tia totient a lui Euler\index{Euler L.}. Func'tia se noteaz'a cu $\varphi$ 'si num'ar'a num'arul de factori relativi primi cu $n$ mai mici ca $n$. Spre exemplu, pentru $n=12$ avem factori relativ primi $1$, $5$, $7$ 'si $11$ deoarece $(1,12)=1$\footnote{where $(m, n)$ is $gcd(m,n)$ that is the greatest common divisor of $n$ and $m$}, $(5,12)=1$, $(7,12)=1$ 'si $(11,12)=1$, deci $\varphi(12)=4$. 'In acest capitol sunt enumerate c\^{a}teva din propriet'a'tiile acestei func'tii. Deasemenea s-a generat fi'sierul $\varphi.prn$ care con'tine valorile func'tiei $\varphi$ pentru $n=1,2,\ldots,10^6$. Tot 'in acest capitol se prezint'a o generalizare a teoremei lui Euler\index{Euler L.} referitoare la func'tia totient $\varphi$ 'si algoritmul de determinare a perechi $(s,m_s)$ care verific'a ecua'tia diofantic'a $a^{\varphi(m_s)}\equiv a^s\md{m}$, unde $a,m\in\Ns$. 
Euler\index{Euler L.}'s totient function also known as the $\varphi$ function that counts the natural numbers less than or equal to $n$ that are relatively prime is described in Chapter four. As an example, for $n=12$ the relatively prime factors are $1$, $5$, $7$, and $11$ because $(1,12)=1$\footnote{where $(m, n)$ is $gcd(m,n)$ that is the greatest common divisor of $n$ and $m$}, $(5,12)=1$, $(7,12)=1$, and $(11,12)=1$, thus $\varphi(12)=4$. The chapter also describes the most important properties of this function. The latter section of the chapter contain the algorithm that generates the file $\varphi.prn$ that contains the values of the function $\varphi$ for $n$ raging from $1,2,\ldots,10^6$. Also, in this chapter the describes a generalization of Euler\index{Euler L.} theorem relative to the totient function $\varphi$ and the algorithm the computes the pair $(s,m_s)$ that verifies the Diophantine equation $a^{\varphi(m_s)}\equiv a^s\md{m}$, where $a,m\in\Ns$. 

%In chapter 5 we define a function $L$ which will allow us to (separately or simultaneously) generalize many theorems from Number Theory obtained by Wilson\index{Wilson D.}, Fermat\index{Fermat P.}, Euler\index{Euler L.}, Gauss\index{Gauss C. F.}, Lagrange\index{Lagrange J. L.}, Leibniz\index{Leibniz G.}, Moser\index{Moser L.}, and Sierpinski\index{Sierpinski W.}.
In chapter 5 we define a function $L$ which will allow us to (separately or simultaneously) generalize many theorems from Number Theory obtained by Wilson\index{Wilson D.}, Fermat\index{Fermat P.}, Euler\index{Euler L.}, Gauss\index{Gauss C. F.}, Lagrange\index{Lagrange J. L.}, Leibniz\index{Leibniz G.}, Moser\index{Moser L.}, and Sierpinski\index{Sierpinski W.}.

%Capitolul 6 este dedicat rezolv'arii analitice a unor ecua'tii diofantice ca: ecua'tia liniar'a cu 2 necunoscute, ecua'tia liniar'a cu $n$ necunoscute, sisteme liniare, ecua'tia de ordinul $n$ cu o necunosct'a, ecua'tia generalizat'a a lui Pell\index{Pell J.} 'si ecua'tia $x^2-2y^4=1$. 'In toate aceste situa'tii s-a prezentat proceduri de calcul simbolic care asigur'a determinarea automat'a a solu'tiilor ecua'tiilor diofantice particulare. Pentru fiecare procedur'a de calcul simbolic s-a rezolvat cel pu'tin un exemplu nebanal.
Various analytical solutions to Diophantine equations such as:the second degree equation, the linear equation with $n$ unknown, linear systems, the $n$ degree equation with one unknown, Pell\index{Pell J.} general equation, and the equation $x^2-2y^4=1$. For each of this cases, in chapter six we present symbolic computation that ensure the detection of the solutions for the particular Diophantine equations.

Chapter seven describes the solutions to over  $60~\eta$--Diophantine equations with a specific search domains. By doing so, we obtain a partial solution to each of this equations. Each section contains the search domain and the solutions along side the execution times.

The Conclusions and Index section conclude the book.




==> Introducere_engl.tex <==
\chapter{Introduction}

A linear Diophantine equation is an equation of the form $ax+by=c$
where $a,b,c\in\Int$ and the solutions $x$and $y$ are integers.
These equations can be completely solved using the well known
algorithm developed by Brahmagupta\index{Brahmagupta}
\citep{WeissteinDiophantineEquation}.

In 1900 Hilbert\index{Hilbert D.} wondered whether a more general
algorithm for solving the linear Diophantine equations couldn't be
provided. It is well known that such an algorithm doesn't exist
for the first order solution of a Diophantine equation, a
statement that was proven by
\cite{Matiyasevich1970}\index{Matiyasevich Y. V.}.


The function $\eta$ associates to each natural number $n$ the
smallest natural number $m$ which has the property that $m$ is a
multiple of $n$. In this book we aim to solve, either analytically
or empirically, Diophantine and $\eta$--Diophantine (i.e.
Diophantine equations involving the function $\eta$ of
\cite{Smarandache1980a}\index{Smarandache F.}).

By an analytical method of solving an equation we mean providing a
general solution for the Diophantine equation which completely
solves the problem. For example, the equation $a\cdot x-b\cdot
y=c$, where $a,b,c\in\Ns$, has the general solution $x_k=b\cdot
k+x_0$ and $y_k=a\cdot k+y_0$, where $(x_0,y_0)$ is a particular
solution for the equation and $k$ is an integer,
$k\ge\max\set{\lceil-x_0/b\rceil,\lceil-y_0/a\rceil}$.

By an empirical method of solving an equation we mean a set of
algorithms (or programs) which provide the solutions for the
Diophantine equation in a bounded network of points of integer
coordinates called by us $d$--dimensional \emph{search domain}.
For example, for the $\eta$--Diophantine equation $\eta(m\cdot
x+n)=x$ on a possible $d=3$--dimensional \emph{search domain}l,
the solutions may be the triplets $(m,n,x)\in
D_c=\set{1,2,\ldots,1000}\times\set{1,2,\ldots1000}\times\set{1,2,\ldots,999}$.

The first chapter contains sections covering prime numbers,
primality tests, prime factorization algorithms for natural
numbers, methods for counting prime numbers up to a number
$x\in\Real$. All these are necessary for solving
$\eta$--Diophantine equations using the empirical method.

In the second chapter the $\eta$ function is defined and its
properties known up to today are given. These are necessary in
order to present the \cite{Kempner1918}\index{Kempner A. J.}
algorithm for calculating the $\eta$ function. At the end of this
chapter we provide the command sequence used to generate the file
$\eta.prn$ which contains the values of $\eta(n)$ for
$n=1,2,\ldots,10^6$.

The third chapter contains a presentation of divisor functions
$\sigma_0$, $\sigma_1$, (usually the notation $\sigma$ is used to
denote $\sigma_1$), $\sigma_2$ ' and $s$. The function
$\sigma_0(n)$ counts the number of divisors of $n$. The value of
$\sigma(n)=\sigma_1(n)$ is equal to the sum of $n$'s divisors. The
value of $\sigma_2(n)$ is equal to the sum of the second powers of
the divisors of $n$ and, generally, the value of $\sigma_k(n)$ is
the sum of the $k$th power of the divisors of $n$. Divisors of $n$
are considered natural numbers that divide $n$ including $1$ and
$n$ itself [therefore] the proper divisors for $n$ are the
divisors of $n$ excluding $n$ itself. Then the function
$s(n)=\sigma(n)-n$ is, in fact, the sum of the proper divisors. In
addition to these definitions of the functions above, the
properties and computing algorithms for these functions are given.
With the use of these algorithms (computer programs) the files
$\sigma0.prn$, $\sigma1.prn$, $\sigma2.prn$, $s.prn$ containing
all the values of  functions $\sigma_0(n)$, $\sigma(n)$,
$\sigma_2(n)$ and $s(n)$ for $n=1,2,\ldots,10^6$ were generated. A
special section of this chapter was dedicated to the $k$--perfect
numbers.

Chapter 4 treats Euler's\index{Euler L.} totient function denoted
$\varphi$. The function count the number of integers less than $n$
that are relative prime to $n$. For instance, if $n=12$,  $1$,
$5$, $7$ and $11$ are relative prime to $12$ [for?]
$(1,12)=1$\footnote{where $(m, n)$ is $gcd(m,n)$ that is the
greatest common divisor of $n$ and $m$}, $(5,12)=1$, $(7,12)=1$
and $(11,12)=1$, therefore $\varphi(12)=4$. Some of the properties
of this function are enumerated. The file $\varphi.prn$ containing
the values of the function $\varphi$ for $n=1,2,\ldots,10^6$ was
generated. The chapter also contains a generalization for
Euler's\index{Euler L.} theorem on the totient function $\varphi$
and an algorithm for determining a pair $(s,m_s)$ that verifies
the Diophantine equation $a^{\varphi(m_s)}\equiv a^s\md{m}$, where
$a,m\in\Ns$.

In chapter 5 we define a function $L$ which will allow us to
(separately or simultaneously) generalize many theorems from
Number Theory obtained by Wilson\index{Wilson D.},
Fermat\index{Fermat P.}, Euler\index{Euler L.}, Gauss\index{Gauss
C. F.}, Lagrange\index{Lagrange J. L.}, Leibniz\index{Leibniz G.},
Moser\index{Moser L.}, and Sierpinski\index{Sierpinski W.}.

Chapter 6 is dedicated to the analytical method for solving some
Diophantine equation such as: linear equations with 2 variables,
linear equations with $n$ variables, equation of the $n$--th
degree with one variable, linear systems, generalized
Pell's\index{Pell J.} equation and the equation $x^2-2y^4=1$. For
all these situations procedures of symbolic computation ensuring
the automatic determination of solutions of particular types of
Diophantine equations are presented. For each procedure at least
one non trivial example was solved.

Chapter 7 covers methods for solving $\eta$--Diophantine equations
using empiric search on a search domain. The chapter contains a
presentation of search domains, run times for equation solving,
the number of solutions obtained and, obviously the solutions
themselves.

The book ends with a section of conclusions and indexes of names,
of notations and of Mathcad functions used in this volume.

